MC2SleepNet: Multi-modal Cross-masking with Contrastive Learning for Sleep Stage Classification

Sleep profoundly affects our health, and sleep deficiency or disorders can cause physical and mental problems. Despite significant findings from previous studies, challenges persist in optimizing deep learning models, especially in multi-modal learning for high-accuracy sleep stage classification. Our research introduces MC2SleepNet (Multi-modal Cross-masking with Contrastive learning for Sleep stage classification Network). It aims to facilitate the effective collaboration between Convolutional Neural Networks (CNNs) and Transformer architectures for multi-modal training with the help of contrastive learning and cross-masking. Raw single channel EEG signals and corresponding spectrogram data provide differently characterized modalities for multi-modal learning. Our MC2SleepNet has achieved state-of-the-art performance with an accuracy of both 84.6% on the SleepEDF-78 and 88.6% accuracy on the Sleep Heart Health Study (SHHS). These results demonstrate the effective generalization of our proposed network across both small and large datasets.

==> Equation/abbreviated.tex <==
% \begin{align}
% \label{eq20-1}
% \mathcal{L}^{Sg}_{CE} = \mathcal{L}_{recover}(\hat{Y}^{Sg}, Y) \text{, where } 
% \\ \nonumber
% \text{MLP}(t^{Sg}_{i, j}) \in \hat{Y}^{Sg} \text{ for all } t^{Sg}_{i, j} : i \in \{1, \ldots, N\}, j \in \{1, \ldots, L\}
% \end{align}
% \vspace{-15pt}

% \begin{align}
% \label{eq20-2}
% \mathcal{L}^{Sp}_{CE} = \mathcal{L}_{recover}(\hat{Y}^{Sp}, Y) \text{, where } 
% \\ \nonumber
% \text{MLP}(t^{Sp}_{i, j}) \in \hat{Y}^{Sp} \text{ for all } t^{Sp}_{i, j} : i \in \{1, \ldots, N\}, j \in \{1, \ldots, L\}
% %\mathcal{L}^{Sp}_{CE} = \mathcal{L}_{recover}(\text{MLP}(t^{Sp}_{i, j}), Y)  + \mathcal{L}_{unmask}(\text{MLP}(t^{Sp}_{i, k}), y_{i, k}) 
% \end{align}
% \vspace{-15pt}

% \begin{align}
% \label{eq20-3}
% \mathcal{L}^{Sg \oplus Sp}_{CE} = \mathcal{L}_{recover}(\hat{Y}^{SS}, Y) \text{, where } 
% \\ \nonumber
% \text{MLP}(t^{SS}_{i, j}) \in \hat{Y}^{SS} \text{ for all } t^{SS}_{i, j}= t^{Sg}_{i, j} \oplus t^{Sp}_{i, j}, \\ \nonumber
% : i \in \{1, \ldots, N\} \text{ and } j \in \{1, \ldots, L\}
% %\mathcal{L}^{Sg \bigoplus Sp}_{CE} = \mathcal{L}_{recover}(\text{MLP}(t^{Sg \bigoplus Sp}_{i, j}), Y)  \\ \nonumber
% %+ \mathcal{L}_{unmask}(\text{MLP}(t^{Sg \bigoplus Sp}_{i, k}), y_{i, k}) 
% \end{align}
% \vspace{-15pt}


==> Table/table3.tex <==
\begin{table}[h]
\centering
\caption{Model accuracy and model size comparison}
\label{table3}
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{Accuracy} & \textbf{\#Parameters} \\
\hline
XSleepNet & 82.3 & $5.74 \times 10^6$  \\
XSleepNet+TF & 83.1 & $6.20 \times 10^6$\\
MC$^2$SleepNet & 83.5 & $5.76 \times 10^6$  \\
\hline
\end{tabular}
\end{table}

==> Table/table5-2.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{10pt}
\caption{Our proposed methods efficacy analysis. ST: SleepTransformer Backbone, SP: SleePyco Backbone, CL: Contrastive learning pre-training, PT: Pre-training with only label guidence, FT: Fine-tuning, M: Masking predict strategy}
\label{table5}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Method} & \textbf{ACC} & \textbf{MFI} & \textbf{k} \\
\hline
ST (single) & 81.5 & 75.1 & 0.744 \\
\hline
SP (single) & 83.5 & 78.0 & 0.773 \\
\hline
PT (multi) & 83.8 & 77.4 & 0.776 \\
\hline
CL + FT (multi) & 83.7 & 77.8 & 0.775 \\
\hline
PT + M + FT (multi) & 84.5 & 79.1 & 0.786 \\
\hline
CL + M + FT (multi) & 84.7 & 79.5 & 0.788 \\
\hline
\end{tabular}
\end{table}

==> Table/table99.tex <==
\begin{table}[ht]
\centering
\caption{Data Augmentation Pipeline with Signal and Spectrogram}
\label{table6}
\begin{tabular}{lccc}
\hline
\textbf{Transformation Pipeline} & \textbf{Min} & \textbf{Max} & \textbf{ACC} \\
\hline
Amplitude Scaling & 0.5 & 2 & \\
Time Shift & -300 & 300 & \\
Amplitude Shift (\(\mu V\)) & -10 & 10 & \\
Zero-masking (samples) & 0 & 300 & 0.5 each \\
Additive Gaussian Noise (\(\sigma\)) & 0 & 0.2 & \\
Band-stop Filter & 0.5 & 30.0 & \\
\hline
\end{tabular}
\end{table}

